Revisiting Unsupervised Learning for Defect Prediction

Collecting quality data from software projects can be time-consuming and expensive. Hence, some researchers explore "unsupervised" approaches to quality prediction that does not require labelled data. An alternate technique is to use "supervised" approaches that learn models from project data labelled with, say, "defective" or "not-defective". Most researchers use these supervised models since, it is argued, they can exploit more knowledge of the projects. At FSE'16, Yang et al. reported startling results where unsupervised defect predictors outperformed supervised predictors for effort-aware just-in-time defect prediction. If confirmed, these results would lead to a dramatic simplification of a seemingly complex task (data mining) that is widely explored in the software engineering literature. This paper repeats and refutes those results as follows. (1) There is much variability in the efficacy of the Yang et al. predictors so even with their approach, some supervised data is required to prune weaker predictors away. (2)Their findings were grouped across $N$ projects. When we repeat their analysis on a project-by-project basis, supervised predictors are seen to work better. Even though this paper rejects the specific conclusions of Yang et al., we still endorse their general goal. In our our experiments, supervised predictors did not perform outstandingly better than unsupervised ones for effort-aware just-in-time defect prediction. Hence, they may indeed be some combination of unsupervised learners to achieve comparable performance to supervised ones. We therefore encourage others to work in this promising area.

==> Makefile <==
Src=unsuper#
Bib=$(shell ls *.bib)#
D=$(HOME)/tmp/$(Src)#

define grab
   gs -sDEVICE=pdfwrite -dNOPAUSE -dBATCH -dSAFER \
       -dFirstPage=$(1) -dLastPage=$(2) \
       -sOutputFile=$@ $<
endef

all: dirs tex bib  tex tex tex     done

typo:
	- git status
	- git commit -am "typo"
	- git push origin master

commit:
	- git status
	- git commit -a
	- git push origin master

update:
	- git pull origin master

status:
	- git status

one: dirs tex done 

open:
	open $(D).pdf


skim:
	defaults write -app Skim SKAutoReloadFileUpdate -boolean true 
	/Applications/Skim.app/Contents/MacOS/Skim $(D).pdf &


view:
	evince $(D).pdf &

abe :  $(D)_a.pdf $(D)_b.pdf $(D)_e.pdf

$(D).pdf : $(Src).tex $(Bib)
	pdflatex -output-directory=$(HOME)/tmp $(Src)

$(D)_a.pdf : $(D).pdf; $(call grab,1,1)		
$(D)_b.pdf : $(D).pdf; $(call grab,2,16)		
$(D)_e.pdf : $(D).pdf; $(call grab,18,28)		

done: embedfonts  abe
	@printf "\n\n\n==============================================\n"
	@printf       "see output in $(D).pdf\n"
	@printf       "==============================================\n\n\n"
	@printf "\n\nWarnings (may be none):\n\n"
	grep arning $D.log

dirs: 
	- [ ! -d $(HOME)/tmp ] && mkdir $(HOME)/tmp

tex: files $(D).pdf

files:
	cp *.tex $(HOME)/tmp

embedfonts:
	@ gs -q -dNOPAUSE -dBATCH -dPDFSETTINGS=/prepress -sDEVICE=pdfwrite \
          -sOutputFile=$(D)-embedded.pdf $(D).pdf
	@ mv  $(D)-embedded.pdf $(D).pdf

bib:
	echo $(Bib)
	- cp $(Bib) $(HOME)/tmp; cd $(HOME)/tmp; bibtex $(Src)
clean:
	rm $D.*


==> old/1.introduction.tex <==
\section{Introduction}

Defect prediction for software projects has been well studied 
over the past decade and lots of researchers focus on proposing new techniques to improve predictors' performance
or make predictors more feasible for practical situation~\cite{lessmann2008benchmarking,hassan2009predicting,fu2016tuning,graves2000predicting,menzies2007data,hall2012systematic,nagappan2005use,jiang2013personalized,kim2007predicting,kim2008classifying,jing2014dictionary,lee2011micro,moser2008comparative,nam2013transfer,wang2016automatically,yang2016effort,kamei2013large}. 
Traditional defect prediction studies build learners at the granularity of  modules or files level~\cite{lessmann2008benchmarking,menzies2007data,nam2013transfer,wang2016automatically,fu2016tuning,hall2012systematic}, which can be
used to identify whether the file or module has defects after applying prediction models. 
Even though learners
may have very high accuracy, it still requires a lot of efforts from quality assurance team 
to inspect each predicted file~\cite{kamei2013large} or
module and it also adds much difficulty to fix the defects since 
the owner of the related files might not be available ~\cite{anvik2006should} or the owner forgets 
details of the implementation~\cite{weiss2007long}. 

To address these problems, researchers proposed to build defect prediction learners on change level~\cite{kim2008classifying,mockus2000predicting,sliwerski2005changes,shihab2012industrial} and predict the defect-inducing changes at check-in time~\cite{kamei2013large,fukushima2014empirical,yang2016effort}. This type of just-in-time(JIT) defect prediction
has the following benefits over traditional counterpart~\cite{kim2008classifying,kamei2013large}:
\bi
\item Predict defects at a fine granularity: Compared to the whole file or module, a committed change includes small amount of codes, which will dramatically reduce the efforts for inspection if it is predicted as defective.
\item Predict defects in a timely manner: Traditional defect prediction usually happens after the software or the package is completed. However, JIT defect prediction could happen as soon as the change is committed, which
will make the defect fixed easily as the developer would still remember the details about the change.
\ei

Mockus et al.~\cite{mockus2000predicting} conduct the first study to predict defects on change metrics from a telecommunication software project, whereas Kim et al.~\cite{kim2008classifying} further evaluate the effectiveness of change metrics on 12 open source projects.
Shihab et al.~\cite{shihab2012industrial} designed a logistic regression model to predict the risk change on
industrial software. They find that  features, like lines of code added
by the change and the developer experience, are strongly correlated to risk change. To take the effort into account, Kamei et al.~\cite{kamei2013large}
used a modified linear regression to build an effort-ware JIT defect predictor.
They reported that with $20\%$ of the total effort required to inspect all the changes,
their method can identify $35\%$ of all the defect-inducing changes. Yang et al.~\cite{yang2016effort} argued
that data collection for training models is time consuming and 
building supervised learners is expensive. Therefore, they
proposed to build unsupervised learners directly on testing data~\cite{yang2016effort}.
In their study, they identify 12 different change metrics and build
12 unsupervised learners accordingly. Based on their evaluation results, they claimed that many unsupervised learners perform better than Kamei et al.'s supervised learner~\cite{yang2016effort}. However, since the unsupervised learners
are built on the testing data, to deploy unsupervised learners on actual software
project, we still have the following questions:
\bi 
\item Do all the $12$ unsupervised learners perform equally well so that we can randomly pick one and apply to future projects?
\item If not, without any prior knowledge on the future project,  which unsupervised learner we have to use?
\ei

According to our best knowledge, Yang et al. did not shed lights on these issues in ~\cite{yang2016effort}. Therefore, in this paper, we empirically study how to make such
simple unsupervised learners work on actual software projects. Specifically, we set the following research questions:

\bi 
\item \textbf{RQ1:Do all simple unsupervised learners perform better than the best supervised learner?}\\
Experimental results show that not all, actually only two unsupervised learners,  outperform than the best supervised learner for only two evaluation measures. This indicates that without any prior knowledge on the performance of unsupervised learners, we can't find randomly pick an supervised learner to apply. Based on this observation, we proposed a new supervised learner, {\it OneWay}.

\item \textbf{RQ2:Does {\it OneWay} perform  better than unsupervised learners?}\\
Experimental results show that {\it OneWay} has pretty stable and good performance on all data sets for all evaluation measures. When deploying to the actual software projects, it performs better than unsupervised learners on average for effort-aware JIT defect prediction. 

\item \textbf{RQ3:Does {\it OneWay} perform  better than supervised learners?} \\
Experimental results {\it OneWay} performs significantly better than all 4 supervised learners in terms of {\it Recall} and $P_{opt}$, but not for {\it Precision}.
\ei

The rest of this paper is organized as follows. Section 2 describes the background and related work on defect prediction.
Section 3 explains the effort-ware JIT defect prediction methods investigated in this study, while Section 4 describes the
experimental settings of our study, including research questions that motivate our study, data sets and experimental design.
Section 5 presents the results. Section 6 discusses the threats to the validity of our study. Section 7 concludes the paper.




==> old/2.relatedwork.tex <==
\section{Background and Related Work}

\subsection{Traditional Defect Prediction}
In traditional defect prediction, we measure the complexity of
software project using McCabe metrics, Halstead's effort metrics and  CK object-oriented code mertics~\cite{kafura1987use,chidamber1994metrics,mccabe1976complexity,halstead1977elements} at
a coarse granularity, like file or package level. It usually happens after the project has completed. With the collected data instances as well as the corresponding labels(defective or non-defective), we can  build defect prediction models using supervised machine learning algorithms such as Decision Tree, Random Forests, SVM, Naive Bayes and Logistic Regression\cite{khoshgoftaar2001modeling,khoshgoftaar2003software,khoshgoftaar2000balancing,menzies2007data,lessmann2008benchmarking,hall2012systematic}. After that, such trained defect predictor can be applied
to predict the defects on future projects. This type of defect prediction, where training data and testing data are from the same project, is referred as within-project defect prediction(WPDP).

However, for a new software project or a project with limited historical data, researchers
proposed to conduct cross-project defect prediction(CPDP), where the training data is from a different software project with the same metric measured as the testing project. Turhan et al. proposed the nearest neighbor method for CPDP~\cite{turhan2009relative}, where the most similar
training data to the testing data is select for building the model. However the performance of this method is still worse than WPDP. Transfer learning  techniques were proposed  in ~\cite{nam2013transfer, ma2012transfer}, both of these techniques achieve comparable performance with WPDP. Zhang et al.~\cite{zhang2014towards} proposed to build a universal model instead of building models
for each individual target project. They cluster projects based on the similarity of the distribution of 26 predictors, and derive the rank transformations using quantiles of predictors for a cluster. In this way, this universal model was fitted on data sets from 1398 open source projects. Their results show that the universal model obtains prediction performance comparable to WPDP models~\cite{zhang2014towards}. Recently, Nam et al.~\cite{nam2015clami} have proposed
to use unsupervised learning methods, CLA and CLAMI, for defect prediction  on unlabeled data sets. The key idea of
the CLA/CLAMI approaches is to label an unlabeled data set by using the magnitude of metric values~\cite{nam2015clami}. The intuition of this method is based on the empirical observation that higher complexity causes more defect-proneness~\cite{menzies2007data,rahman2013and}. They report that CLA/CLAMI acheive 0.636 and 0.723 F1-measure and AUC, respectively. 

To make defect prediction more feasible in practice, Nam et al.~\cite{nam2015heterogeneous}consider a situation where the data extracted from the
target project has different sets of metrics from any available training data. In this case,
current techniques for CPDP are difficult to apply across projects with heterogeneous metric sets. They proposed a  heterogeneous defect prediction method, which conducts metric selection and metric matching to build a prediction model between projects with heterogeneous metric sets. Experimental results  from 28 subjects show that about $68\%$ of predictions outperform or are comparable to WPDP with statistical significance~\cite{nam2015heterogeneous}.


\subsection{Just-In-Time Defect Prediction}
In traditional defect prediction has some drawbacks such as prediction at a coarse granularity and started at very late stage of software development circle~\cite{kamei2013large},wheras in JIT defect prediction paradigm, the models use change metrics generated from each change as the predictors, which
could easily help developers to narrow down the code for inspection and JIT defect prediction could be conducted right before developers commit the change. JIT defect prediction becomes more practical method for practitioners to carry out.

Mockus et al.~\cite{mockus2000predicting} conduct the first study to predict 
software failures on 5ESS software updates(a telecommunication system)
by using logistic regression on 
data sets consisted of change metrics of the project. Kim et al.
further evaluate the effectiveness of change metrics  on open source projects in ~\cite{kim2008classifying}, where they propose to apply support vector machine to build a defect predictor based on software change metrics, where they achieved $78\%$ accuracy and $60\%$ recall on average.Since the training data might
not available when building the defect predictor, Fukushima et al.~\cite{fukushima2014empirical} introduced
cross-project models into JIT defect prediction. Their results showed that using data from other projects to build JIT defect predictor is feasible. 

However, all the previous JIT defect prediction studies do not consider the efforts required to inspect the predicted defect-introducing changes. Kamei et al.~\cite{kamei2013large} take the effort into account and conduct a large-scale study on the effectiveness of JIT defect prediction, where they claim that using $
20\%$ of efforts required to inspect all changes, their modified linear regression model could
detect $35\%$ defect-introducing changes. Inspired by Menzies et al's ManualUp model(i.e., small size of modules inspected first)~\cite{menzies2010defect}, Yang et al. propose to build $12$ unsupervised learners by sorting the reciprocal values of $12$ different change metrics on each testing data set in descendant order. They
report that the experimental results from six open source projects
show that with $20\%$ efforts, many
unsupervised learners perform better than the state-of-art supervised learner.

Yang et al.'s method is so simple and might benefit a lot for defect prediction if working properly. However, there some issues
when applying to actual project. Firstly, since these unsupervised learners are built directly on testing data set, this indicates that there is no way to tell which learner(s) will perform better than supervised learners or all of them work equally same. 
If all of these learners have similar performance, then we have a strong confidence to select only one, instead of all of them, to apply on future projects. Otherwise, there should be a way to figure out which learner to select. Secondly, in yang's study, they only evaluate learners for two evaluation measures and there is no way to show how these unsupervised
learners perform in terms of different evaluation measures. Without any training data, how could we believe that those learners would meet our evaluation goals. Unfortunately, Yang et al. did not consider these issues in their work~\cite{yang2016effort}. 








==> old/3.method.tex <==
\section{Method}


\begin{table}[!htp]
\caption{Change Metrics Used in Our Defect Data Sets.}\label{tab:CM}
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|l}
\hline
\rowcolor{lightgray}
Metric & Description  \\\hline
NS & Number of modified subsystems~\cite{mockus2000predicting}.\\
ND & Number of modified directories~\cite{mockus2000predicting}. \\
NF & Number of modified directories~\cite{nagappan2006mining}. \\
Entropy & Distribution of the modified code across each file~\cite{d2010extensive,hassan2009predicting}.\\\hline
LA & Lines of code added~\cite{nagappan2005use}.\\
LD & Lines of code deleted~\cite{nagappan2005use}.\\
LT & Lines of code in a file before the current change~\cite{koru2009investigation}.\\\hline
FIX & Whether or not the change is a defect fix~\cite{guo2010characterizing,yin2011fixes}. \\\hline
NDEV & Number of developers that changed the modified files~\cite{matsumoto2010analysis}. \\
AGE & The average time interval between the last and the current \\
    & change~\cite{graves2000predicting}. \\
NUC & The number of unique changes to the modified files~\cite{d2010extensive,hassan2009predicting}. \\ \hline
EXP & The developer experience in terms of number of changes~\cite{mockus2000predicting}.\\
REXP & Recent developer experience~\cite{mockus2000predicting}. \\
SEXP & Developer experience a the subsystem~\cite{mockus2000predicting}. \\\hline

\end{tabular}}
\end{table}

\subsection{Unsupervised Learner} \label{unsupervised}
In this section, we describe the effort-aware 
just-in-time(JIT) unsupervised defect learner proposed by Yang et al. \cite{yang2016effort},
which serves as a baseline method in this study.

As described by Yang et al.\cite{yang2016effort},  their simple unsupervised
 defect learner is built on change metrics, which is shown in \tab{CM}. These
 14 different change metrics can be divided into 5 dimensions\cite{kamei2013large}:
 \bi
 \item Diffusion: NS, ND, NF and Entropy.
 \item Size: LA, LD and LT.
 \item Purpose: FIX.
 \item History: NDEV, AGE and NUC.
 \item Experience: EXP, REXP and SEXP.
 \ei 
The {\it diffusion} dimension characterizes how a change is 
distributed at different levels of granularity.
As discussed by Kamei et al.~\cite{kamei2013large},
a highly distributed change is harder to keep track
and more likely to introduce defects. The {\it size} dimension
characterize the size of a change, where it's believed that
the software size is positively related to defect proneness
~\cite{nagappan2005use,koru2009investigation}. Yin et al.~\cite{yin2011fixes}
report that the bug-fixing process can also introduce new bugs. 
Therefore, the {\it Fix} metric could be used as a defect evaluation metric.
The {\it History} dimension includes some historical information
about the change, which has been proven to be a good defect indicator.
For example, Matsumoto et al. ~\cite{matsumoto2010analysis} find that the files
previously touched by many developers are likely to contain more defects.
The {\it Experience} dimensions describe the experience of software programmers
for the current change because Mockus et al.~\cite{mockus2000predicting} show that
more experienced developers are less likely to introduce a defect. More details
about these metrics can be found in ~\cite{kamei2013large}.

In Yang et al.'s study, for each change metric $M$, 
they build an unsupervised learner that ranks all the changes
based on the corresponding value of $\frac{1}{M(c)}$in descendant order, 
where $M(c)$ is the value of the selected change metric for each change $c$.
Therefore, the changes with smaller change metric values will ranked higher.
Totally, for each project, there will be 12 simple
unsupervised learners~(LA and LD are excluded), 
 
 
%  The literature show that these factors perform well to in defect prediction
% \cite{mockus2000predicting,nagappan2006mining,nagappan2005use,
% koru2009investigation, hassan2009predicting,guo2010characterizing,
% matsumoto2010analysis,graves2000predicting,d2010extensive,kamei2013large}. 
% In particular, Kamei et al.\cite{kamei2013large}

\subsection{Supervised Learner}
To further evaluate the unsupervised learner, we selected some supervised learners
that already used in Yang et al.'s work. 

As reported in both Yang et al.'s~\cite{yang2016effort}
and Kamei et al.'s~\cite{kamei2013large} work, linear regression model (EALR) outperforms
all other supervised learners for effort-aware JIT defect prediction.
For the linear regression learner, instead of predicting $Y(x)$,
we predict $\frac{Y(x)}{Effort(x)}$, where $Y(x)$ indicates whether this change
is a defect or not($1$ or $0$) and $Effort(x)$ represents the effort required 
to inspect this change. Note that this is the same method to 
build EALR as Kamel et al. ~\cite{kamei2013large}.

In defect prediction literature, KNN, J48 and Random Forests methods are simple 
yet widely used to as defect learners and have been proven to perform, if not best, quite
well~\cite{lessmann2008benchmarking,menzies2007data,hall2012systematic}. These three
learners are also used in Yang et al's study. For these
supervised learners, $Y(x)$ was used as the dependant variable. 
For KNN method, we set $K=8$. To fully reproduce
Yang et al.'s results,  all the settings in this paper strictly follow
their work~\cite{yang2016effort} without further explanation.


\subsection{OneWay Learner}\label{OneWay}
% \wei{The following text probabily need to move to motivation part}


As described in section \ref{unsupervised}, given a new project,
Yang et al.'s unsupervised method actually builds 12
learners for each project according to each predictor(change metric).
However, without using some validation data and ground truth labels to test,
we don't know which simple unsupervised learner works well for this project.
Generally, there are two situations need to consider, where

\bi
\item all 12 learners actually perform better than supervised learners.
\item or only some learners actually perform better than supervised learners.
\ei

In the first situation, we have the confidence that there's no need to
care about choosing which change metric to build unsupervised learners on.
Simply choosing one out of those 12 metrics and building a simple
learner on it will work quite well for JIT effort-aware defect prediction. 
However, in the second situation, we have to come up a way to
figure out how to select good predictors. Otherwise, randomly selecting
one feature to build an unsupervised learner won't guarantee the performance.
In other words, without any training data or supervised data, we can't even
tell which situation fits our new project.


Actually, based on our our preliminary experiment results
shown in the following section, for those six projects
investigated by Yang et al, some of those 12 unsupervised
learners do perform worse than supervised learners. 
That means we can't say which simple unsupervised learner actually
works for the new project before doing testing. In this case,
we need to select the proper metric to build unsupervised learner.



To make simple unsupervised learner actually work in practice,
we propose {\it OneWay} learner, which is supervised learner built on
the idea of simple unsupervised learner. The pseudocode for OneWay
is shown in Algorithm~\ref{alg:OneWay}. In the following description,
We use the superscript numbers to denote the line number of pseudocode. 

The general idea of {\it OneWay} is to use the best metric obtained
from the supervised feature pruning process to build a single feature
unsupervised learner. Specifically, {\it OneWay} firstly builds simple
unsupervised learners for each metric on training data$^{L3-L4}$, then
evaluate each of those learners in terms of evaluation metrics$^{L5-L6}$,
like Popt, ACC, Precision and F. After that, if the desirable
evaluation goal is set, the metric which performs best on the corresponding
evaluation goal is returned as the best metric; otherwise, the metric
which gets the highest mean score over all evaluation metrics is returned$^{L13-L22}$.
Finally, a simple unsupervised learner like Yang et al's. is built only
on such best metric$^{L10}$.




 
\begin{algorithm}[!htp]
\small
\caption{Pseudocode for OneWay}
\begin{algorithmic}[1]
\Require $\mathit{data\_train}$, $\mathit{data\_test}$, $\mathit{eval\_goal} \in \{\mathit{F,Popt,ACC,Precision,...}\}$
\Ensure $\mathit{result}$
\vspace{2mm}
\Function{OneWay}{$\mathit{data\_train}$, $\mathit{data\_test}$, $\mathit{eval\_goal}$}
  \State $\mathit{all\_scores} \gets$ NULL
  \For{$\mathit{metric}$ in $\mathit{data\_train}$}
      \State $\mathit{learner}\gets$ buildUnsupervisedLearner($\mathit{data\_train}$, $\mathit{metric}$)
      \State $\mathit{scores} \gets $evaluate($\mathit{learner}$)\\
      \quad \qquad //$\mathit{scores}$ include all evaluation goals, e.g., $\mathit{Popt,ACC,...}$
      \State $\mathit{all\_scores}$.append($\mathit{scores}$)
  \EndFor
  \State $\mathit{best\_metric} \gets$ pruneFeature($\mathit{all\_scores}$, $\mathit{eval\_goal}$)
  \State $\mathit{result} \gets$ buildUnsupervisedLearner($\mathit{data\_test}$, $\mathit{best\_metric}$)
  \State \Return $\mathit{result}$
\EndFunction
\Function{pruneFeature}{$\mathit{all\_scores}$, $\mathit{eval\_goal}$}
  \If{$\mathit{eval\_goal}$ == NULL}
    \State $\mathit{ mean\_scores} \gets$ getMeanScoresForEachMetric($\mathit{all\_scores}$)
    \State $ \mathit{best\_metric} \gets$ getMetric(max($\mathit{mean\_scores}$)) 
    \State \Return $\mathit{best\_metric}$
   \Else
     \State $\mathit{best\_metric} \gets$ getMetric(max($\mathit{all\_scores[``eval\_goal"]}$))
     \State\Return $\mathit{best\_metric}$
  \EndIf
\EndFunction
\end{algorithmic}
\label{alg:OneWay}
\end{algorithm}






==> old/4.experiment_design.tex <==
\section{Experimental Settings}

\subsection{Research Questions}
To further investigate how unsupervised learners work for 
Effort-Aware JIT defect prediction in practice and its limitations,
whether {\it OneWay} method perform better compared to unsupervised learners and traditional
supervised learners, we set the following research questions:
\bi 
\item Do all simple unsupervised learners perform better than the best supervised learners?
\item Does {\it OneWay} perform  better than unsupervised learners?
\item Does {\it OneWay} perform  better than supervised learners?
\ei

When reading the results from Yang et al~\cite{yang2016effort},
we find that they report the performance scores of each learner across all projects in one chart, which might miss some information about how each learner perform on each project. Are these unsupervised learners working consistently across all the project data? if not, how it might look like? Therefore, we want to investigate the RQ1 in this study firstly.

Another observation is that even though Yang et al. propose that 
simple unsupervised learners could work better than supervised learners for effort-aware defect prediction, they actually ignore the fact that it's hard to know which metric actually works for the defect prediction before testing their unsupervised learners except for the case where all the metrics work perfectly. Based on this fact, we propose a new method, {\it OneWay}, which is simple yet applicable to practical effort-ware
JIT defect prediction scenario. Therefore,
in RQ2 and RQ3, we want to evaluate how well our proposed {\it OneWay} method perform compared to the unsupervised learners and supervised learners.

Considering our goals and questions, we reproduce Yang et al's results
and report for each project to answer RQ1 and For RQ2 and RQ3, we implement our {\it OneWay}
methods, and compare it with unsupervised learners and supervised learners on different projects in terms of various evaluation metrics.

\subsection{Data Sets}
In this study, we conduct our experiment on the data sets
from six well-known open source projects, Bugzilla, 
Columba, Eclipse JDT, Eclipse Platform, Mozilla and PostgreSQL.
These data sets are shared by Kamei et al.~\cite{kamei2013large},
which are the same data sets used in Yang et al.'s study~\cite{yang2016effort}.
The statistics of the data sets are listed in ~\tab{datasets}.
From ~\tab{datasets}, we know that all these six data sets
cover at least 4 years historical information, and the longest one is PostgreSQL, 
which includes 15 years data. The total changes for these six data sets
are from 4620 to 98275, which are sufficient for us to conduct
empirical study. In this study, if a change introduces one or more defect then
this change is considered as defect-introducing change. The percentage of 
defect-introducing changes ranges from 5\% to 36\% and over all, the average
modified files per change for all six projects is around 4.

\begin{table}[]
    \centering
    \caption{Statistics of the Studied Data Sets}
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{@{}c|c c c c c@{}}
    \hline
        \multirow{3}{*}{Project} &
        \multirow{3}{*}{Period} & 
        \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Total\\ Change\end{tabular}} & 
        \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}$\%$ of \\ Defects \end{tabular}} &
        \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Avg LOC \\ per \\ Change\end{tabular}}  &
        \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}} \# Modified \\ Files per\\ Change\end{tabular}} \\ \\  \\\hline
    Bugzilla & 08/1998 - 12/2006 & 4620 & 36\% & 37.5 & 2.3 \\
    Platform & 05/2001 - 12/2007 & 64250 & 14\%& 72.2 & 4.3 \\
    Mozilla & 01/2000 - 12/2006 & 98275 & 5\% & 106.5 & 5.3 \\
    JDT & 05/2001 - 12/2007 & 35386 & 14\% & 71.4 & 4.3 \\
    Columba & 11/2002 - 07/2006 & 4455 & 31\% & 149.4 & 6.2 \\
    PostgreSQL & 07/1996 - 05/2010 & 20431 & 25\% & 101.3 & 4.5 \\ \hline
    \end{tabular}}
    \label{tab:datasets}
\end{table}



\subsection{Experimental Design}\label{exp_design}

When applying data mining algorithms to build predictive models,
one important principle is not to test on the data used in training. 
There are many ways to design a experiment that satisfies this principle.
However, some of those methods have limitations. For example, 
leave-one-out is too slow for large data sets and cross-validation mixes up older and newer data
(such that data from the past may be used to test on future data). 

To avoid these problems, we used the time-wise-cross-validation method in~\cite{yang2016effort},
which will be easier for us to compare our results against theirs.
(Due to the space limitation,
we don't provide the cross-project prediction results in this paper).
The following experiment design ensure that the testing data was actually
created after traning data.
Firstly, we sort all the changes in each project based on the commit date. 
Then all the changes that submitted in the same month are grouped together.
For a given project data set that covers totally $N$ months history, when building
a defect predictor,
\bi 
\item The two consecutive months data,  $i$ and $i+1$, are used as the training data, which will be used
to train supervised learners and {\it OneWay} learner.
\item The other two months data, $i+4$ and $i+5$, which are
two months later than the training data was created, are used as
the testing data to test the supervised learners and {\it OneWay} learner.
\ei

By using this method, each training and testing data set
has two months data, which will include sufficient positive and negative instances
for the supervised learners to learn. For any project that includes $N$ months data,
we can perform $N-5$ different experiments to evaluate our learners when $N$ is greater than 5.
For all the unsupervised learners, only the testing data 
is used to build the model and evaluate the performance.

To statistically compare the differences between {\it OneWay} 
with supervised and unsupervised learners,
we use 
% Scott-Knott procedure recommended by \cite{mittas2013ranking}.
% Scott-Knott first looks for a break in the sequence that maximizes the expected
%     values in the difference in the means before and after the break.
%     More specifically,  it  splits $l$ values into sub-lists $m,n$ in order to maximize the expected value of differences  in the observed performances before and after divisions. E.g. for lists $l,m,n$ of size $ls,ms,ns$ where $l=m\cup n$, Scott-Knott divides the sequence at the break that maximizes:
%      \[E(\Delta)=\frac{ms}{ls}abs(m.\mu - l.\mu)^2 + \frac{ns}{ls}abs(n.\mu - l.\mu)^2\]
% Scott-Knott then applies some statistical hypothesis test $H$ to check if $m,n$ are significantly different.
% If so, Scott-Knott then recurses on each division; 
% Otherwise, Scott-Knott terminates and returns the ranks
% of sub-lists.
Wilcoxon single ranked test is applied to compare
the performance scores of the learners in this study. As in~\cite{yang2016effort},
to control the false discover rate, the Benjamini-Hochberg(BH) adjusted p-value 
is used to test whether two distributions are statistically significant
at the level of $0.05$~\cite{benjamini1995controlling}. 
To measure the effect size of performance scores among {\it OneWay} and supervised/unsupervised learners,
we compute Cliff's $\delta$ that is a non-parametric effect size measure~\cite{romano2006exploring}.
As Romano et al. suggested, we evaluate the magnitude of the effect size as follows:
negligible ($|\delta|<0.147$ ), small ($ 0.147<|\delta|<0.33$), medium ($0.33<|\delta|<0.474$ ), and large (0.474 $\leq|\delta|$)~\cite{romano2006exploring}.


\begin{figure}[!t]
    \centering
    \includegraphics[width=.47\textwidth]{pic/delta.pdf}
    \caption{Example of an effort-based cumulative lift chart for Bugzilla~\cite{kamei2013large}.}
    \label{fig:delta}
\end{figure}
\subsection{Evaluation Measures}

For effort-aware defect prediction, in addition to evaluate how learners correctly predict a defect-introducing change, we have to take account of the efforts that required to inspect prediction. Ostrand et al.~\cite{ostrand2005predicting}
report that given a project, $20\%$ files contain on average $80\%$  of all defects in the project.
Although nothing magical about the number $20\%$, it has been used as a cutoff
value to set the efforts required for the defect inspection when evaluating the defect learners ~\cite{yang2016effort,kamei2013large,mende2010effort,monden2013assessing}.
That is, given $20\%$ effort\footnote{Effort means total number
of files/codes that predicted as defective need to inspect in the project}, 
how many defects actually can be detected by the learner.
To be consistent with Yang et al, in this study, we restrict our efforts to $20\%$ of total efforts.

To evaluate the performance of effort-aware JIT defect
prediction learners in our study, 
we used the following 4 metrics: {\it Precision, Recall, F1-score} and $P_{opt}$,
which are widely used in defect prediction literature~\cite{menzies2007data,menzies2010defect,zimmermann2007predicting, kamei2013large,yang2016effort,monden2013assessing}.

\vskip 2ex
\begin{eqnarray}\nonumber
Precision &=& \frac{True \, Positive}{True \, Positive +False \, Positive}\\ \nonumber
Recall &=& \frac{True \, Positive}{True \, Positive +False \, Negative}\\ \nonumber
F1 &=& \frac{2*Precision*Recall}{Recall + Precision}
\end{eqnarray}
where {\it Precision} denotes the percentage of actual defective changes to all the predicted changes and {\it Recall} is the percentage of predicted defective changes to all actual defective changes. {\it F1 } is a measure that combines both {\it precision} and {\it Recall} which is the harmonic mean of {\it Precision} and {\it Recall}. As mentioned above, we use $20\%$ efforts to evaluate learners, which means
we only inspect $20\%$ of all the top ranked changes that are predicted as defective. Therefore, all the evaluation metrics, {\it Precision}, {\it Recall} and {\it F1} considered in the following sections are using $20\%$ efforts.  

The last evaluation metric used in this study is $P_{opt}$,
which is defined as $1- \Delta_{opt}$, where $\Delta_{opt}$ is the area
between the effort(code-churn-based) cumulative lift charts of the optimal
model and the prediction model (shown in \fig{delta}). 
In this chart, the x-axis is considered as the percentage of required effort to inspect the change and the y-axis
is the percentage of defect-introducing change found in the selected change. In the optimal model, all the changes are sorted by the actual defect density in descendant order, while for the predicted model, all the changes are sorted by 
the actual predicted value in  descendant order.

According to \cite{yang2016effort,kamei2013large,monden2013assessing}, the normalized $P_{opt}$ can be denoted as follows:
\begin{eqnarray} \nonumber
P_{opt}(m) = 1- \frac{S(optimal)-S(m)}{S(optimal)-S(worst)}
\end{eqnarray}
where $S(optimal)$, $S(m)$ and $S(worst)$ represent the area of the optimal model, predicted model, and worst model
in \fig{delta}, respectively. Note that the worst model is built by sorting all the changes according to the actual defect density in ascendant order, which is used to normalize $P_{opt}$. Since the value of normalized $\Delta_{opt}$ is in $[0,1]$, then the normalized $P_{opt}$ is also in $[0,1]$. Therefore, for any learner, it performs better than random predictor only if the ${P_{opt}}$ is greater than 0.5

As similar to the above three evaluation metrics, {\it Precision, Recall, F1-score}, we use $20\%$ of all effort when computing $P_{opt}$, which is consistent to Yang et al.'s work~\cite{yang2016effort}. Note that in this study, in addition to $P_{opt}$ and $ACC$(it's actually recall) that used in Yang et al's work\cite{yang2016effort}, we include 
$Precision$ and $F1$ measures and they provide more insights about all the learners evaluated in the study from very different perspectives, which will be shown in the next section.






==> old/5.results.tex <==
\section{Empirical Results}
In this section, we present the experimental results to investigate how
simple unsupervised learners work in practice and evaluate the performance
of the proposed method, {\it OneWay}, compared with supervised and unsupervised learners.

Before we start off, we need a sanity check to see if we can fully 
reproduced Yang et al.'s results in ~\cite{yang2016effort}. Since 
there might be some details missed in boxplot figures, we prefer to
compare performance scores. In~\cite{yang2016effort}, Yang et al.
provide the median values of $P_{opt}$ and $Recall$ for the EALR
model and the best two simple unsupervised models, LT and AGE, from
time-wise cross evaluation. Therefore, we use those numbers to check
our results. Note that only EALR and unsupervised learners need to implement from scratch,
where some differences might introduce if not 
properly follow Yang et al.'s work~\cite{yang2016effort}.

\begin{table}[]
    \centering
    \caption{ Comparison in $P_{opt}$: Yang's method(A) vs. Our implementation(B)}
    % \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l|c c| c c| c c}

    \hline
        \multirow{2}{*}{Project} &
        \multicolumn{2}{c|}{EALR} &
        \multicolumn{2}{c|}{LT} &\multicolumn{2}{c}{AGE} \\
        \cline{2-7}
        &A & B& A&B&A&B \\
        \hline
        Bugzilla & 0.59 & 0.59 &0.72 &  0.72& 0.67  & 0.67 \\
        Platform & 0.58 & 0.58 & 0.72 & 0.72 & 0.71 & 0.71\\
        Mozilla & 0.50 &0.50 &0.65 &0.65 &0.64&0.64\\
        JDT & 0.59 & 0.59& 0.71 &0.71 & 0.68  & 0.69\\
        Columba & 0.62 & 0.62& 0.73 & 0.73 & 0.79  & 0.79 \\
        PostgreSQL & 0.60 &0.60&0.74&0.74&0.73 &0.73\\ \hline
        Average & 0.58 & 0.58 & 0.71 & 0.71 & 0.70 &0.70 \\ \hline
    \end{tabular}
    % }
    \label{tab:comp_Popt}
\end{table}



\begin{table}[]
    \centering
    \caption{Comparison in $Recall$ : Yang's method(A) vs. Our implementation(B)}
    % \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l|c c| c c| c c}
    \hline
        \multirow{2}{*}{Project} &
        \multicolumn{2}{c|}{EALR} &
        \multicolumn{2}{c|}{LT} &\multicolumn{2}{c}{AGE} \\
        \cline{2-7}
        &A & B& A&B&A&B \\
        \hline
        Bugzilla & 0.29 & 0.30 &0.45 &  0.45& 0.38  & 0.38 \\
        Platform & 0.31 & 0.30 & 0.43 & 0.43 & 0.43 & 0.43\\
        Mozilla & 0.18 &0.18 &0.36 &0.36 &0.28&0.28\\
        JDT & 0.32 & 0.34& 0.45 &0.45 & 0.41  & 0.41\\
        Columba & 0.40 & 0.42& 0.44 & 0.44 & 0.57  & 0.57 \\
        PostgreSQL & 0.36 &0.36&0.43&0.43&0.43 &0.43\\ \hline
        Average & 0.31 & 0.32 & 0.43 & 0.43 & 0.41 & 0.41 \\ \hline
    \end{tabular}
    % }
    \label{tab:comp_Recall}
\end{table}


As shown in \tab{comp_Popt} and \tab{comp_Recall}, for unsupervised learners,
LT and AGE, we get the exactly same performance scores on all projects in terms
of {\it Reall} and ${\it P_{opt}}$. This is reasonable because unsupervised learners
are very straightforward and easy to implement. For the supervised learner, EALR, 
these two implementations do not have differences in ${\it P_{opt}}$, while the maximum
difference in  {\it Recall} is only ${0.02}$. Since the differences are quite small,
then we believe that our implementation reflect the details about EALR and unsupervised
learners in~\cite{yang2016effort}. 

For other supervised learners used in this study, like {\it J48, IBk}, and {
\it RandomForest}, we use the same algorithms from Weka package and set the same parameters as in~\cite{yang2016effort}.

\textbf{RQ1: Do all simple unsupervised learners perform better than the best supervised learner?}


To answer this question, we build 4 supervised learners and 12
unsupervised learners on the six project data sets using incremental learning
method as described in Section~\ref{exp_design}. 
% For each project, every 6 consecutive
% months data is used for one experiment, where the first 2 months  data are used train
% the supervised defect learners and the last two 2 months data is used as 
% the test data to evaluate the performance for both supervised and unsupervised learners.


\fig{sup_unsup} shows the boxplot of {\it Recall}, {\it $P_{opt}$}, {\it F1} and {\it Precision} for
supervised learners and unsupervised learners on 6 data sets. For each learner, the boxplot shows the
25th percentile, median and 75 percentile  values for one data set. The horizontal dashed lines indicate
the median of best supervised learners, which is to help visualize the median differences between unsupervised
learners and supervised learners.  


\begin{figure*}[!htbp]
\begin{center}
    \includegraphics[width=.45\textwidth,height=2.8in]{pic/hist-cv-tw-Sup-Unsup-ACC.pdf}\includegraphics[width=.45\textwidth,height=2.8in]{pic/hist-cv-tw-Sup-Unsup-Popt.pdf}
    \includegraphics[width=.45\textwidth,height=2.8in]{pic/hist-cv-tw-Sup-Unsup-F1.pdf}\includegraphics[width=.45\textwidth,height=2.8in]{pic/hist-cv-tw-Sup-Unsup-PREC.pdf}
\caption{Performance comparisons among supervised and unsupervised learners over 6 projects(from top to bottom are  bugzilla, platform, mozilla, jdt, columba, postgres). } 
\label{fig:sup_unsup}
\end{center}
\end{figure*}

The colors of the box indicate
the significant difference between learners. The blue color represents that the corresponding learner
is significantly {\it better} than the best supervised learner according to Wilcoxon signed-rank, where the
BH corrected p-value is less than 0.05 {\it and} the magnitude of the difference between these two learners is NOT trivial
according to Cliff's delta, where $|\delta| \geq 0.147$. The black color represents that the corresponding learner is not significantly {\it better} than the best supervised learner {\it or} the magnitude of the difference between these two learners is trivial, where $|\delta| \leq 0.147$. The red color represents that the corresponding learner is significantly {\it worse} than the best supervised learner {\it and} the  magnitude of the difference between these two learners is NOT trivial.

From \fig{sup_unsup},  we can clearly see that not all unsupervised
learners perform statistically better than the best supervised learner
across all different evaluation metrics. Specifically, for {\it Recall}, 
on one hand, there are only $\frac{2}{12}$,
$\frac{3}{12}$, $\frac{6}{12}$, $\frac{2}{12}$, $\frac{3}{12}$ and $\frac{2}{12}$ of
total unsupervised learners perform statistically {\it better} than
the best supervised learner on 6 data sets, respectively.
On the other hand, there are $\frac{6}{12}$, $\frac{6}{12}$, $\frac{4}{12}$, $\frac{6}{12}$,
$\frac{5}{12}$ and $\frac{6}{12}$ of
total unsupervised learners perform statistically {\it worse} than the best supervised learner on 6 data sets, respectively. This indicates that (1) about $50\%$ unsupervised learners actually 
perform worse than the best supervised learner on any data set;
(2) without any prior knowledge,  we can't even know which
unsupervised learner(s) actually work on the test data. The similar trend as {\it Recall}
can be found in $ P_{opt}$ as well.


For {\it F1}, our observation is that only LT on bugzilla and AGE on postgres
 perform statistically better than the best supervised learner. 
 Other than that, no unsupervised learner performs better on any data set. Furthermore, surprisingly,
 no unsupervised learner works significantly better than the best supervised learner on any 
data sets in terms of {\it Precision}. As we can see,{\it RandomForest} perform well on all six data sets.
This suggests that unsupervised learners have very low
precision for effort-ware JIT defect prediction and can't be deployed to the business situation where 
demanding a high precision.



\begin{figure*}[htbp]
\begin{center}
 \includegraphics[width=.45\textwidth,height=3in]{pic/hist-cv-tw-Unsup-OneWay-ACC.pdf}\includegraphics[width=.45\textwidth,height=3in]{pic/hist-cv-tw-Unsup-OneWay-Popt.pdf}
 \includegraphics[width=.45\textwidth,height=3in]{pic/hist-cv-tw-Unsup-OneWay-F1.pdf}\includegraphics[width=.45\textwidth,height=3in]{pic/hist-cv-tw-Unsup-OneWay-PREC.pdf}
\caption{Performance comparisons between the proposed {\it OneWay} learner and unsupervised learners over 6 projects(from top to bottom are  bugzilla, platform, mozilla, jdt, columba, postgres).}
\label{fig:unsup_oneway}
\end{center}
\end{figure*}


Overall, for a given data set, no one specific unsupervised learner works 
better than the best supervised learner across all evaluation
metrics; For a given evaluation measure, most unsupervised learners
didn't perform better across all data sets.
There are two exceptions, LT and AGE for both {\it Recall} and ${P_{opt}}$. 
But, we know that after evaluating all the learners with the ground truth.
Before, the unsupervised learning nature won't allow us know anything about the learner's performance.
The above results indicate that:

\vskip 1ex
 \begin{myshadowbox}
    Not all simple unsupervised learners perform better than supervised learners for each project and for different evaluation measures.
 \end{myshadowbox}

\textbf{RQ2: Does {\it OneWay} perform  better than unsupervised learners?}

To answer this question, we compare {\it OneWay} learner with 12
unsupervised learners. All these learners are tested on on the six project data 
sets using the same experiment scheme as we did in RQ1.


\begin{figure*}[htbp]
\begin{center}
 \includegraphics[width=.25\textwidth,height=3in]{pic/hist-cv-tw-Sup-OneWay-ACC.pdf}\includegraphics[width=.25\textwidth,height=3in]{pic/hist-cv-tw-Sup-OneWay-Popt.pdf}\includegraphics[width=.25\textwidth,height=3in]{pic/hist-cv-tw-Sup-OneWay-F1.pdf}\includegraphics[width=.25\textwidth,height=3in]{pic/hist-cv-tw-Sup-OneWay-PREC.pdf}
\caption{Performance comparisons between the proposed {\it OneWay} learner and supervised learners over 6 projects(from top to bottom are  bugzilla, platform, mozilla, jdt, columba, postgres).}
\label{fig:sup_oneway}
\end{center}
\end{figure*}

\fig{unsup_oneway} shows the boxplot for the performance distribution of
unsupervised learners and the proposed
{\it OneWay} learner on 6 data sets across 4 evaluation measures. The horizontal 
dashed line denotes the median value of {\it OneWay}. Firstly, according to {\it Recall},
only one unsupervised learner, LT, outperforms {\it OneWay} in $\frac{4}{6}$ data sets. However, {\it OneWay}
significantly outperform$\frac{9}{12}$, $\frac{9}{12}$, $\frac{9}{12}$, $\frac{10}{12}$,
 $\frac{8}{12}$ and $\frac{10}{12}$ of total unsupervised learners on 6 data sets, respectively.
 This observation indicates that {\it OneWay} works significantly better 
 than almost all learners on all 6 data sets in terms of {\it Recall}.
 
 Similarly, we observe that only LT learner works better than {\it OneWay} in
$\frac{3}{6}$ data sets in terms of {\it $P_{opt}$} and AGE outperforms {\it OneWay} only on platform data set.
For the remaining experiments, {\it OneWay} perform better than all the other learners(usually,9 out of 12 learners). In addition, according to {\it F1}, only three unsupervised learners EXP/REXP/SEXP 
perform better than {\it OneWay} on mozilla data set and
LT learner just perform as well as {\it OneWay} and does not have any advantage over{\it OneWay}. The same finding can be observed in {\it Precision} measure.

To get more insights, \tab{unsu_oneway} provides the median values of the best unsupervised learner with {\it OneWay}
for each evaluation measure on all 6 data sets. In that table, for each evaluation measure,
the number in blue background indicates that the best unsupervised learner has a large advantage
over {\it OneWay} according to the cliff's Delta; Similarly, the light blue background means moderate advantage
and the gray background means small advantage. 

From \tab{unsu_oneway}, we observe that in total 24 experiments on all evaluation measures, 
none of these best unsupervised learners outperform {\it OneWay} with a large advantage according
to the cliff's Delta. Specifically,  according to {\it Recall} and $P_{opt}$,
even though LT outperforms {\it OnWay} on four and three data sets, respectively. However, all of
these advantage are small. Meanwhile, REXP and EXP have a moderate improvement
over {\it OneWay} on one and two data sets for {\it F1} and {\it Precision}, respectively.
In terms of the average scores, the maximum magnitude of the difference between the best unsupervised 
learner and {\it OneWay} is $0.02$. In other words, {\it OneWay} is comparable with the best unsupervised
learners on all data sets for all evalution measures.




\begin{table}[]
    \centering
    \caption{Best Unsupervised Learner(A) vs. OneWay(B)}
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l|c c| c c| c c| c c}
    \hline
        \multirow{2}{*}{Project} &
        \multicolumn{2}{c|}{{\it Recall}} &
        \multicolumn{2}{c|}{$P_{opt}$} &
        \multicolumn{2}{c|}{{\it F1}} &
        \multicolumn{2}{c}{{\it Precision}}\\
        \cline{2-9}
        &A(LT) & B & A(LT)&B&A(REXP)&B &A(EXP)&B \\
        \hline
        Bugzilla &\colorbox{gray!50}{0.45} & 0.36 &\colorbox{gray!50}{0.72} &  0.65& 0.33  & 0.35 & 0.40 & 0.39  \\
        Platform & \colorbox{gray!50}{0.43} & 0.41 & \colorbox{gray!50}{0.72} & 0.69 & 0.16 & 0.17 &\colorbox{gray!50}{0.14} &0.11\\
        Mozilla & \colorbox{gray!50}{0.36} &0.33 &\colorbox{gray!50}{0.65} &0.62 &\colorbox{blue!20}{0.10}&0.08 &\colorbox{blue!20}{0.06} &0.04\\
        JDT & \colorbox{gray!50}{0.45}& 0.42& 0.71 & 0.70  & 0.18 & 0.18 &\colorbox{blue!20}{0.15} &0.12\\
        Columba & 0.44& 0.56 & 0.73 & 0.76 & 0.23 & 0.32 &0.24 &0.25\\
        PostgreSQL & 0.43 &0.44&0.74&0.74&0.24 & 0.29 &\colorbox{gray!50}{0.25} &0.23\\ \hline
        Average & 0.43 &0.42 &0.71& 0.69 & 0.21 & 0.23 &0.21 &0.19\\ \hline
    \end{tabular}
    }
    \label{tab:unsu_oneway}
\end{table}


Overall, we find that (1) no one unsupervised learner significantly
outperform {\it OneWay} on all data sets for a given evaluation measure;(2)usually, {\it OneWay}
works as well as the best unsupervised learner and has significant better performance than almost
all unsupervised learners on all data sets for all evaluation measures. Therefore, the above results suggest:
\vskip 1ex
 \begin{myshadowbox}
    As a simple supervised learner, {\it OneWay} has pretty stable and good performance on
    all data sets for all evaluation measures and
    it performs  better than unsupervised learners for effort-aware JIT defect prediction. 
 \end{myshadowbox}


\textbf{RQ3: Does {\it OneWay} perform  better than supervised learners?}

To answer this question, we compare {\it OneWay} learner with 4
supervised learners, including EALR, Randomforest, J48 and IBk. 
EALR is considered to be the state-of-art learner for effort-aware
JIT defect prediction and all the other three learners are widely used 
in defect prediction literature over past years. We evaluate all these
learners on the six project data 
sets using the same experiment scheme as we did in RQ1.


From \fig{sup_oneway}, we have the following observations. Firstly, 
the performance of {\it OneWay} is significantly better than all
these four supervised learners in terms of {\it Recall} and ${P_{opt}}$
on all 6 data sets. Also, EALR works better than Randomforest, J48 and IBk,
which is consistent to Kamei et al's finding~\cite{kamei2013large}. Secondly,
according to {\it F1}, randomforest and IBk perform slightly better than {\it OneWay}
in 2 out of 6 data sets. For most cases, {\it OneWay} has a similar performance
to these supervised learners and there is no much difference between them. However,
when reading {\it Precision} scores, we find that, in most cases, supervised
learners perform significantly better than {\it OneWay}. Specifically, Randomforest,
J48 and IBk outperform {\it OneWay} on all data sets and EALR is better on 3 data sets. 
This finding is consistent to the observation in RQ1 where all unsupervised learners
perform worse than supervised learnrs. Since {\it OneWay} is built on the idea of
unsupervised learners, it explains why {\it OneWay} does worse in {\it Precision}.
As an aside, EALR is never
the best supervised learner in any case, but it's still better or simiar to {\it OneWay}.

\begin{table}[]
    \centering
    \caption{Best Supervised Learner(A) vs. OneWay(B)}
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l|c c| c c| c c| c c}
    \hline
        \multirow{2}{*}{Project} &
        \multicolumn{2}{c|}{{\it Recall}} &
        \multicolumn{2}{c|}{$P_{opt}$} &
        \multicolumn{2}{c|}{{\it F1}} &
        \multicolumn{2}{c}{{\it Precision}}\\
        \cline{2-9}
        &A(EALR) & B & A(EALR)&B&A(IBk)&B &A(RF)&B \\
        \hline
        Bugzilla & 0.30 & 0.36 &0.59 &  0.65& 0.30  & 0.35 & \colorbox{blue!50}{0.59} & 0.39  \\
        Platform & 0.30 & 0.41 & 0.58 & 0.69 & \colorbox{blue!20}{0.23} & 0.17 &\colorbox{blue!50}{0.38} &0.11\\
        Mozilla & 0.18 &0.33 &0.50 &0.62 &\colorbox{blue!50}{0.18}&0.08 &\colorbox{blue!50}{0.27} &0.04\\
        JDT & 0.34& 0.42& 0.59 & 0.70  & \colorbox{gray!50}{0.22} & 0.18 &\colorbox{blue!50}{0.31} &0.12\\
        Columba & 0.42& 0.56 & 0.62 & 0.76 & 0.24 & 0.32 &\colorbox{blue!50}{0.50} &0.25\\
        PostgreSQL & 0.36 &0.44&0.60&0.74&0.21 & 0.29 &\colorbox{blue!50}{0.69} &0.23\\ \hline
        Average & 0.32 &0.42 &0.58& 0.69 & 0.23 & 0.23 &0.46 &0.19\\ \hline
    \end{tabular}
    }
    \label{tab:unsup_oneway}
\end{table}

From \tab{unsup_oneway},  we have the following observation.
First of all, the maximum  difference in median values between 
EALR and {\it OneWay} is from $0.15$ and $0.14$, which are $83\%$ and $23\%$ improvements
over $0.18$ and $0.60$ on mozilla and postgreSQL data sets in terms of {\it Recall} and ${P_{opt}}$.
For both measures, {\it OneWay} improve the average scores by $0.1$ and $0.11$, which are
$31\%$ and $19\%$ improvement over EALR. Secondly, according to {\it F1}, IBk outperform
{\it OneWay}  on three data sets with a large, moderate and small advantage, respectively.
The largest difference in median is $0.1$. Finally, as we discuss before, the best 
supervised learner for {\it Recall}, RandomForest, have very large advantage over
{\it OneWay} on all data sets. The largest difference is $0.46$.


Overall, we conclude that (1) given one project data, no one supervised learner works
better than {\it OneWay} for all evaluation measures;(2) {\it OneWay} outperforms all
4 supervised learners in terms of {\it Recall} and $P_{opt}$, respectively. but it performs
significantly worse than Randomforest, J48 and IBk. Therefore, our answer to RQ3 is:
\vskip 1ex
 \begin{myshadowbox}
    {\it OneWay} performs significantly better than all 4 supervised learners in terms of {\it Recall}
    and $P_{opt}$, but not for {\it Precision}.
 \end{myshadowbox}












==> old/5.results211.tex <==
\section{Empirical Results}


\begin{figure*}[htbp]
\begin{center}
    \includegraphics[width=.45\textwidth,height=3.0in]{pic/hist-cv-tw-Sup-Unsup-ACC.pdf}\includegraphics[width=.45\textwidth,height=3.0in]{pic/hist-cv-tw-Sup-Unsup-Popt.pdf}
    \includegraphics[width=.45\textwidth,height=3.0in]{pic/hist-cv-tw-Sup-Unsup-F1.pdf}\includegraphics[width=.45\textwidth,height=3.0in]{pic/hist-cv-tw-Sup-Unsup-PREC.pdf}
\caption{Performance comparisons among supervised and unsupervised learners over 6 projects(from top to bottom are  bugzilla, platform, mozilla, jdt, columba, postgres). } 
\label{default}
\end{center}
\end{figure*}


\begin{figure*}[htbp]
\begin{center}
 \includegraphics[width=.4\textwidth,height=3in]{pic/hist-cv-tw-Unsup-OneWay-ACC.pdf}\includegraphics[width=.4\textwidth,height=3in]{pic/hist-cv-tw-Unsup-OneWay-Popt.pdf}
 \includegraphics[width=.4\textwidth,height=3in]{pic/hist-cv-tw-Unsup-OneWay-F1.pdf}\includegraphics[width=.4\textwidth,height=3in]{pic/hist-cv-tw-Unsup-OneWay-PREC.pdf}
\caption{default}
\label{default}
\end{center}
\end{figure*}


\begin{figure*}[htbp]
\begin{center}
 \includegraphics[width=.2\textwidth,height=3in]{pic/hist-cv-tw-Sup-OneWay-ACC.pdf}\includegraphics[width=.2\textwidth,height=3in]{pic/hist-cv-tw-Sup-OneWay-Popt.pdf}\includegraphics[width=.2\textwidth,height=3in]{pic/hist-cv-tw-Sup-OneWay-F1.pdf}\includegraphics[width=.2\textwidth,height=3in]{pic/hist-cv-tw-Sup-OneWay-PREC.pdf}
\caption{default}
\label{default}
\end{center}
\end{figure*}



==> old/6.discussion.tex <==
\section{Discussion}
\subsection{ Is a Low Precision {\it OneWay} Learner Useful}
\wei{DO we need to use precision? how to explain. feel struggled here.}


In last section, we notice that {\it OneWay} learner does not 
perform well in terms of {\it Precision} compared to the supervised learners
in RQ3. However, it is still a quite useful learner and the reason is as follows.

First of all, for effort-ware defect prediction like this study, we only set 
 $20\%$ efforts(measured in code churn) as our budget, which is quite small amount
 of effort compared with the total. 




 






\subsection{Threats to Validity}
In this section, we discuss the potential factors that might threat our results.

\textbf{Internal Validity}. The internal validity is related to uncontrolled
aspects that may affect the experimental results. One threat to the interval
is how well our implementation of unsupervised learners could represent 
the Yang et al.'s method. To mitigate this thread, we strictly follow 
the approach described in Yang et al's work and test our implementation on the
same data sets as in \cite{yang2016effort}. By comparing the performance
scores, we find that our implementation can generate the same results. Therefore,
we believe we can avoid this threat.

\textbf{External Validity}. The external validity is related to the
possibility to generalize our results. Our observations and conclusions
from this study may not be generalized to other software projects. In this study,
we use six widely used open source software project data as the subject.
As all these software projects are written in java, we can't  guarantee that
our findings can be directly generalized to other projects,
specifically to the software that implemented in other programming
languages. Therefore, the future work might include verify our findings on 
other software project.

In this work, we used the data sets from~\cite{yang2016effort,kamei2013large}, where
totally 14 features were extracted from the software projects.  We build and test the
{\it OneWay} learner on those features as well. However, there might be some other features
that not measured in these data sets that work well as indicators for defect prediction.
For example, the role of the developer who committed the change(e.g., owner of the files,or not),
functionality of the the files modified in this change(e.g., core functionality or not).
Those new features that not explored in this study might improve the performance of 
our {\it OneWay} learner.


==> old/7.conclusion.tex <==
\section{Conclusion and Future Work}

In this paper, we revisit Yang et al.'s work~\cite{yang2016effort}
about using unsupervised learners for effort-ware just-in-time 
defect prediction and find that not all unsupervised learners
work better than supervised learners on 6 data sets for different evaluation
measures. This suggests that we can't randomly pick any one unsupervised learner
to perform effort-ware defect prediction and it's necessary to figure out
how to pick the best metric(s) even before building the unsupervised learner.
Therefore, we propose a supervised learner, {\it OneWay}, which automatically
selects the potential best one metric to build a simple learner with training data.
Our results indicate that, 
\bi
\item in terms of {\it Recall}, $P_{opt}$ and {\it F1},
{\it OneWay} outperforms all most unsupervised learners and supervised learners
on 6 data sets. The largest improvement is $83\%$ over EALR. 
\item it is not doing very well for {\it Precision}.
\ei
Since there are many domains and applications where a high-recall-and-low-precision
learner is required, therefore, we believe that {\it OneWay} can be deployed for practical
purpose.

This study opens the new reserach direction of applying simple supervised 
techniques to perform the defect prediction. As shown in this
study as well as Yang et al.'s work~\cite{yang2016effort}, instead of using
traditional machine learning algorithms like J48 and Randomforest, simply sorting
data according to one metric can be a good defect predictor model, at least for
effort-ware just-in-time defect prediction. Therefore, we recommend the future
defect prediction research should more focus on simple techniques.

For the future work, we plan to extend this study on other software projects,
especially those developed by the other programming languages. After that,
we plan to investigate some new change features to see if that helps improve
{\it OneWay}'s performance.





